Unifying Motion Deblurring and Frame Interpolation with Events

Slow shutter speed and long exposure time of frame-based cameras often cause visual blur and loss of inter-frame information, degenerating the overall quality of captured videos. To this end, we present a unified framework of event-based motion deblurring and frame interpolation for blurry video enhancement, where the extremely low latency of events is leveraged to alleviate motion blur and facilitate intermediate frame prediction. Specifically, the mapping relation between blurry frames and sharp latent images is first predicted by a learnable double integral network, and a fusion network is then proposed to refine the coarse results via utilizing the information from consecutive blurry inputs and the concurrent events. By exploring the mutual constraints among blurry frames, latent images, and event streams, we further propose a self-supervised learning framework to enable network training with real-world blurry videos and events. Extensive experiments demonstrate that our method compares favorably against the state-of-the-art approaches and achieves remarkable performance on both synthetic and real-world datasets.

==> Figs-Fig-Feasibility.tex <==
\begin{figure}[th]
    \centering
        \includegraphics[width=0.9\linewidth]{Figs-imgs-Feasibility.jpg}
        \caption{Example of three overlapped blurry frames, where the target timestamp $t_0$ locates inside the exposure time of $B_{01}$ and $B_{02}$, but outside the exposure time of $B_{12}$.}
        \label{Feasibility}
\end{figure}




% \begin{figure}[!t]
%   \centering
%   \begin{subfigure}{1\linewidth}
%     \centering
%         \includegraphics[width=0.85\linewidth]{Figs/imgs/Feasibility.jpg}
%         \caption{Three overlapped blurry frames}
%         \label{Feasibility}
%     \end{subfigure}
    
    
%   \begin{subfigure}{1\linewidth}
%   \centering
%         \includegraphics[width=1\linewidth]{Figs/imgs/PreExample.jpg}
%         \caption{Example of pre-processing}
%         \label{PreExample}
%     \end{subfigure}

%   \caption{ (a)Example of joint deblurring and interpolation. (b) Preprocessing Example}
% \end{figure}

==> Figs-Fig-NetDetail.tex <==
\begin{figure}[th]
    \centering
        \includegraphics[width=\linewidth]{Figs-imgs-NetDetail.jpg}
        \caption{Detailed architecture of our LDI and fusion networks, where $C_{in}, C_{out}$ indicate the channel of input and output tensors, respectively. }
        \label{fig:NetDetail}
\end{figure}

==> Figs-Fig-ProbState.tex <==
\begin{figure}[!t]
  \centering
%   \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
  \includegraphics[width=1\linewidth]{Figs-imgs-ProbState.jpg}

   \caption{Illustration of blurry video enhancement. Motion Deblurring task aims at restoring the sharp latent images within the exposure time of blurry frames, and frame interpolation task generally predicts the intermediate latent images between two reference frames. The goal of blurry video enhancement is to reconstruct clear latent images located both inside and between blurry frames, achieving joint deblurring and interpolation.}
   \label{ProbState}
\end{figure}

==> Figs-Figure-psnrloss.tex <==
\begin{figure}[!t]
  \centering
%   \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
    \begin{subfigure}{0.23\textwidth}
    \centering
        \includegraphics[width=\textwidth]{Figs-imgs-loss.png}
        \caption{Training loss}
        \label{loss}
    \end{subfigure}
    \begin{subfigure}{0.23\textwidth}
    \centering
        \includegraphics[width=\textwidth]{Figs-imgs-psnr.png}
        \caption{Training PSNR}
        \label{psnr}
    \end{subfigure}
    \vspace{-3mm}
   \caption{The recorded loss and PSNR during the training with different combinations of loss functions. }
   \label{psnr_loss}
   \vspace{-3mm}
\end{figure}


==> Tabs-test.tex <==
\begin{table}[]
\begin{tabular}{lllllcccc}
\hline
\multirow{3}{*}{Method}                          & \multicolumn{4}{l}{Single frame prediction}                                                               & \multicolumn{4}{c}{7 frames prediction}                                                                           \\ \cline{2-9} 
                                                 & \multicolumn{2}{l}{GoPro}                           & \multicolumn{2}{l}{HQF}                             & \multicolumn{2}{c}{GoPro}                               & \multicolumn{2}{c}{HQF}                                 \\ \cline{2-9} 
                                                 & \multicolumn{1}{c}{PSNR} & \multicolumn{1}{c}{SSIM} & \multicolumn{1}{c}{PSNR} & \multicolumn{1}{c}{SSIM} & PSNR                       & SSIM                       & PSNR                       & SSIM                       \\ \hline
LEVS                                             & 21.884                   & 0.7304                   & 20.009                   & 0.6406                   & 19.851                     & 0.6525                     & 19.959                     & 0.6870                     \\
EDI \textbackslash{}cite\{pan2019bringing\}      & 21.517                   & 0.7446                   & 20.299                   & 0.7340                   & 20.939                     & 0.7277                     & 19.234                     & 0.7053                     \\
eSL-Net \textbackslash{}cite\{wang2020event\}    & 23.143                   & 0.7813                   & 20.438                   & 0.6017                   & 23.955                     & 0.7578                     & 19.866                     & 0.5851                     \\
LEDVDI \textbackslash{}cite\{jiang2020learning\} & 24.325                   & 0.8286                   & 23.925                   & 0.8231                   & 24.038                     & 0.8248                     & 21.558                     & 0.7355                     \\
RED-Net \textbackslash{}cite\{xu2021motion\}     & 26.795                   & 0.8940                   & 26.094                   & 0.8495                   & 26.302                     & 0.8247                     & 24.368                     & 0.8214                     \\ \hline
Ours-GoPro                                       & 32.002                   & 0.9487                   & 26.209                   & 0.8866                   & 31.255                     & 0.9426                     & 24.414                     & 0.8607                     \\
Ours-GoPro-flow                                  & 30.416                   & 0.9291                   & 25.687                   & 0.8779                   & \multicolumn{1}{l}{30.272} & \multicolumn{1}{l}{0.9300} & \multicolumn{1}{l}{23.917} & \multicolumn{1}{l}{0.8507}
\end{tabular}
\end{table}

